Generalized Hierarchical Bayesian Segmentation with Irregular Designs, Multi-Sequence Hierarchies, and Grouped/Latent-Group Designs

Bayesian change-point and segmentation models provide uncertainty-aware piecewise-constant representations of ordered data, but exact inference is often limited to narrow likelihood classes, single sequences, or index-uniform designs. We present BayesBreak, a modular offline Bayesian segmentation framework that separates local block scoring from global inference: each candidate block supplies a marginal likelihood and any needed moment numerators, while a dynamic program combines these scores to compute posteriors over segment counts, boundaries, and latent signals. For weighted exponential-family likelihoods with conjugate priors, block evidences and posterior moments are available in closed form from cumulative sufficient statistics, enabling exact sum-product inference for p(y|k), p(k|y), boundary marginals, and Bayes regression curves. We distinguish these summaries from the joint MAP segmentation, recovered by a separate max-sum recursion. BayesBreak supports design-aware partition priors for irregular observations, exact pooling across replicates with shared boundaries, and latent-template mixtures with exact EM updates. For non-conjugate GLM blocks, the same DP layer can use deterministic local approximations such as Laplace, variational methods, EP, or quadrature. We prove a posterior-odds stability bound: uniform per-block log-evidence error {\epsilon} perturbs k-odds and boundary-odds by at most (k+k'){\epsilon} and 2k{\epsilon}. Validation includes synthetic recovery, calibration, and scaling experiments, plus four real-data illustrations: well-log geology, array-CGH copy number, equity-return volatility, and CpG-atlas methylation.

==> shared/bibliography/annotated_entries/adamsmackay2007bocpd.tex <==

\paragraph{\texttt{adamsmackay2007bocpd}: \citet{adamsmackay2007bocpd}.}
Adams and MacKay formulate online Bayesian changepoint detection through a recursive posterior over run length. BayesBreak uses this work to delimit its scope: BayesBreak is an offline contiguous-partition method that returns a posterior over segment count, fixed-count boundary marginals, Bayes curves, and a separate joint MAP partition, rather than an online filtering distribution. The source therefore informs the online/offline distinction and potential future streaming comparisons, but it is not treated as evidence for BayesBreak's offline exact-DP claims.


==> shared/bibliography/annotated_entries/auger1989segment.tex <==
\paragraph{\texttt{auger1989segment}: \citet{auger1989segment}.}
Auger and Lawrence develop dynamic-programming algorithms for identifying segment neighborhoods under broad segment-fit criteria, including least squares and maximum likelihood. The paper is part of the classical algorithmic lineage for Bellman-style segmentation and shows that an optimal-partition max-sum recurrence is not itself a BayesBreak contribution. BayesBreak differs by using integrated segment likelihoods in Bayesian recursions for normalization and posterior marginals, while retaining a separate max-sum recursion for the joint MAP partition. The paper is used as algorithmic background rather than as a source for Bayesian posterior calculations.


==> shared/bibliography/annotated_entries/barry1992ppm.tex <==

\paragraph{\texttt{barry1992ppm}: \citet{barry1992ppm}.}
Barry and Hartigan introduce product partition models for changepoint problems, including the cohesion factorization that underlies segment-local prior contributions. This is direct prior art for BayesBreak's factorized partition prior. BayesBreak narrows the setting to ordered contiguous partitions and makes the local prior factorization explicit by separating segment cohesion $c_x(i,j)$ from an interior-boundary hazard $h_x(j)$, both of which preserve dynamic-programming factorization. The source prevents any claim that cohesion priors originate here.


==> shared/bibliography/annotated_entries/barry1993bayesCP.tex <==

\paragraph{\texttt{barry1993bayesCP}: \citet{barry1993bayesCP}.}
Barry and Hartigan develop a Bayesian analysis for changepoint problems using the product-partition framework. BayesBreak cites this paper for the Bayesian changepoint and cohesion lineage, including posterior uncertainty about partitions. The exact BayesBreak delta is not generic Bayesian changepoint inference; it is the generalized exponential-family segment formulation, the collection of posterior quantities computed by the sum-product recursion, the hierarchical extensions, and the separately computed joint MAP partition. The comparison also motivates calibrated novelty language.


==> shared/bibliography/annotated_entries/bernardo1994bayesian.tex <==

\paragraph{\texttt{bernardo1994bayesian}: \citet{bernardo1994bayesian}.}
Bernardo and Smith provide the general Bayesian foundations used to interpret marginal likelihoods, posterior model probabilities, posterior predictive quantities, and decision-relevant uncertainty. In BayesBreak, the book supports the distinction between evidence, posterior summaries, and exported point decisions. It does not supply a changepoint algorithm or validate any archived numerical result. Its role is foundational vocabulary and interpretation, especially where the manuscript separates a posterior over partitions from a joint MAP action.


==> shared/bibliography/annotated_entries/blanchard2021lse.tex <==

\paragraph{\texttt{blanchard2021lse}: \citet{blanchard2021lse}.}
Blanchard, Higham, and Higham analyze stable computation of log-sum-exp and softmax functions. BayesBreak uses these numerical primitives throughout log-domain forward/backward recursions, pooled evidence aggregation, template responsibilities, and normalization checks. The source informs implementation and numerical QA rather than the statistical model. It is particularly relevant where underflow would otherwise turn very small but nonzero partition mass into an apparent hard exclusion.


==> shared/bibliography/annotated_entries/bleakley2011groupfused.tex <==
\paragraph{\texttt{bleakley2011groupfused}: \citet{bleakley2011groupfused}.}
Bleakley and Vert propose the group fused lasso for detecting changepoints shared across multiple one-dimensional signals by penalizing multidimensional total variation. It is a task-relevant frequentist comparator for common structural changes across sequences. BayesBreak differs by integrating sequence-specific segment parameters and, in its strict common-boundary model, multiplying sequence-level segment marginal likelihoods before Bayesian dynamic programming. The methods return different inferential objects, so comparisons must use comparable tuning budgets and distinguish point-estimate agreement from posterior uncertainty.


==> shared/bibliography/annotated_entries/carlin1992hierBayesCP.tex <==

\paragraph{\texttt{carlin1992hierBayesCP}: \citet{carlin1992hierBayesCP}.}
Carlin, Gelfand, and Smith present hierarchical Bayesian changepoint analysis and show how uncertainty and pooling can be represented beyond a single flat partition model. BayesBreak uses this paper to locate its shared and grouped extensions within a broader hierarchical Bayesian lineage. The current exact BayesBreak results apply only where subject-level contributions factor through a common boundary vector or known grouping; richer hierarchical dependence generally requires additional computation. The source therefore informs both motivation and scope limits.


==> shared/bibliography/annotated_entries/corradin2026commonstructural.tex <==

\paragraph{\texttt{corradin2026commonstructural}: \citet{corradin2026commonstructural}.}
Corradin, Danese, KhudaBukhsh, and Ongaro cluster time-dependent observations according to common structural-change locations using a latent random-order representation and Bayesian computation. This is the closest verified work for the broad latent-group narrative. BayesBreak retains only a narrower computational object: a finite collection of deterministic changepoint templates optimized under the explicitly stated criterion in Chapter~\ref{ch:templates}, using auxiliary allocation weights and exact responsibility-weighted max-sum updates. The two models should not be conflated, and no claim of first clustering by shared changepoints remains.


==> shared/bibliography/annotated_entries/dempster1977em.tex <==
\paragraph{\texttt{dempster1977em}: \citet{dempster1977em}.}
Dempster, Laird, and Rubin establish the expectation--maximization algorithm for maximum-likelihood estimation with incomplete data. The BayesBreak latent-template routine uses a responsibility-weighted alternating optimization, but its subject--template quantities are prior-weighted partition scores rather than normalized component densities. The book therefore cites EM as optimization background and describes the routine through its displayed finite objective and Jensen minorization; it does not claim an observed-data finite-mixture likelihood or import identifiability conclusions from mixture theory.


==> shared/bibliography/annotated_entries/denison1998bayesian.tex <==
\paragraph{\texttt{denison1998bayesian}: \citet{denison1998bayesian}.}
Denison, Mallick, and Smith develop automatic Bayesian curve fitting with a joint model for the number and positions of knots in piecewise-polynomial representations and reversible-jump Markov chain Monte Carlo for posterior computation. BayesBreak uses the paper as a contrasting Bayesian model-space and computational lineage rather than as an exact changepoint dynamic-programming reference. The comparison makes BayesBreak's scope precise: its exact recursions require a finite ordered candidate set and segment-factorized marginal likelihoods, and do not subsume arbitrary trans-dimensional curve models.


==> shared/bibliography/annotated_entries/diaconis1979conjugate.tex <==

\paragraph{\texttt{diaconis1979conjugate}: \citet{diaconis1979conjugate}.}
Diaconis and Ylvisaker characterize conjugate priors for exponential families. Their normalizer convention supplies the algebra behind BayesBreak's integrated block evidence: cumulative statistic contributions and cumulative log-partition multipliers update the conjugate hyperparameters, and the evidence is a ratio of normalizers times the powered base measure. BayesBreak extends the presentation with an exposure-aware descriptor $d_t$ and a separately declared power/reliability weight $a_t$ so Poisson exposures and binomial trial counts are not conflated with likelihood tempering.


==> shared/bibliography/annotated_entries/fan2017basic.tex <==

\paragraph{\texttt{fan2017basic}: \citet{fan2017basic}.}
Fan and Mackey's BASIC model addresses simultaneous changepoints across many sequences and includes copy-number and S\&P volatility applications. It is the closest multisequence comparator and overlaps the domains of two BayesBreak case studies. BayesBreak's narrower exact result assumes one common boundary vector and conditionally independent subject contributions whose integrated block evidences multiply. The revised book presents this as a restricted exact pooling regime, not the first Bayesian multisequence changepoint method.


==> shared/bibliography/annotated_entries/fearnhead2006exact.tex <==

\paragraph{\texttt{fearnhead2006exact}: \citet{fearnhead2006exact}.}
Fearnhead gives exact and efficient Bayesian inference for a class of multiple-changepoint models with unknown changepoint count, conditionally independent segments, product-partition structure, and quadratic exact computation. This is the closest foundational work for BayesBreak's sum-product recursion and materially constrains novelty. BayesBreak's contribution is the generalized exponential-family segment formulation, posterior moments and changepoint summaries computed by common recursions, the separate max-sum calculation, irregular-design and multiple-sequence extensions, and the finite latent-group criterion.


==> shared/bibliography/annotated_entries/fearnhead2011dependence.tex <==

\paragraph{\texttt{fearnhead2011dependence}: \citet{fearnhead2011dependence}.}
Fearnhead and Liu develop efficient Bayesian multiple-changepoint analysis when parameters can depend across adjacent segments. BayesBreak's protected exact regime instead assumes that, after integration and declared prior factors, a partition score decomposes into local block contributions. This source marks a clear boundary: dependence across segments is scientifically useful but is not covered by the current exact block API without state augmentation or a different recursion.


==> shared/bibliography/annotated_entries/frick2014smuce.tex <==

\paragraph{\texttt{frick2014smuce}: \citet{frick2014smuce}.}
Frick, Munk, and Sieling develop multiscale changepoint inference with simultaneous error control and confidence statements. SMUCE is a relevant baseline because it emphasizes inferential reliability rather than only point recovery. BayesBreak uses it to design task-matched comparisons for boundary recovery and uncertainty, while recognizing that its posterior probabilities and Bayes curves are not directly equivalent to multiscale confidence sets. Any benchmark must therefore specify the inferential target and calibration criterion.


==> shared/bibliography/annotated_entries/fryzlewicz2014wbs.tex <==

\paragraph{\texttt{fryzlewicz2014wbs}: \citet{fryzlewicz2014wbs}.}
Fryzlewicz introduces wild binary segmentation for efficient multiple-changepoint detection, especially when many changes may occur. It is a computationally attractive point-estimation baseline in the BayesBreak experiments. The source informs scaling and recovery comparisons, but it does not return the same posterior objects as BayesBreak. Archived F1 values computed against BayesBreak MAP boundaries are consequently labeled agreement diagnostics, not independent accuracy or evidence of superiority.


==> shared/bibliography/annotated_entries/green1995rjMCMC.tex <==

\paragraph{\texttt{green1995rjMCMC}: \citet{green1995rjMCMC}.}
Green introduces reversible-jump Markov chain Monte Carlo for Bayesian model determination across spaces of differing dimension. Changepoint models can use this machinery to sample segment count and boundaries without the finite factorization required by exact dynamic programming. BayesBreak cites the work as the principal trans-dimensional Bayesian alternative and uses it to state its own restriction: exactness comes from finite ordered support and local factorization, not from universal Bayesian computation.


==> shared/bibliography/annotated_entries/hutter2006bpcr.tex <==

\paragraph{\texttt{hutter2006bpcr}: \citet{hutter2006bpcr}.}
Hutter derives exact Bayesian regression for piecewise-constant functions, including unknown segment count and boundaries, evidence, break probabilities, error estimates, and a Bayesian regression curve. This is direct closest work for several BayesBreak headline outputs. The revised book therefore does not claim that evidence, boundary probabilities, or a Bayes curve originate with BayesBreak. The remaining contribution is the generalized use of exposure-aware segment sufficient statistics, shared and grouped extensions, separate posterior and joint-MAP calculations, and one implementation of these statistical quantities.


==> shared/bibliography/annotated_entries/jaakkola2000logisticvb.tex <==
\paragraph{\texttt{jaakkola2000logisticvb}: \citet{jaakkola2000logisticvb}.}
Jaakkola and Jordan develop a variational bound for Bayesian logistic models. BayesBreak uses the construction only as an established segment-local approximation option for nonconjugate logistic marginal likelihoods or moments. The approximation is not a BayesBreak contribution, and the source does not supply a uniform segment-error rate for the present changepoint setting. Application of the BayesBreak posterior perturbation result therefore requires a separate, model-specific uniform bound over all reachable segments under explicit parameter, initialization, convergence, and tail conditions.


==> shared/bibliography/annotated_entries/jackson2005optpart.tex <==

\paragraph{\texttt{jackson2005optpart}: \citet{jackson2005optpart}.}
Jackson and coauthors give an algorithm for optimal partitioning of interval data, reinforcing the dynamic-programming lineage for globally optimal segmentations. BayesBreak uses this paper to distinguish an optimal partition computed by max-sum recursion from posterior quantities computed by sum-product recursion. Both routes consume the same local scores, but they answer different questions; marginal boundary modes cannot be substituted for the joint MAP partition.


==> shared/bibliography/annotated_entries/killick2012pelt.tex <==

\paragraph{\texttt{killick2012pelt}: \citet{killick2012pelt}.}
Killick, Fearnhead, and Eckley introduce PELT, a pruned optimization method with linear expected computational cost under stated conditions. PELT is a central efficiency comparator for BayesBreak's worst-case $O(k_{\max}n^2)$ exact posterior engine. The comparison is intentionally asymmetric in output richness: PELT targets a penalized optimal segmentation, whereas BayesBreak also returns evidence, segment-count uncertainty, boundary marginals, and model-averaged curves. Fair evaluation must match objectives and tuning budgets.


==> shared/bibliography/annotated_entries/minka2001ep.tex <==

\paragraph{\texttt{minka2001ep}: \citet{minka2001ep}.}
Minka develops expectation propagation as an approximate Bayesian inference method based on iterative moment matching. BayesBreak treats EP as one possible block-local evidence routine for a nonconjugate family. The revised method makes no routine-wide convergence or accuracy claim: EP must return diagnostics and, where global perturbation claims are desired, a certified error against a trustworthy reference on every reachable block. The source contributes the approximation mechanism, not evidence for BayesBreak-specific rates.


==> shared/bibliography/annotated_entries/muller2011ppmx.tex <==

\paragraph{\texttt{muller2011ppmx}: \citet{muller2011ppmx}.}
M\"uller, Quintana, and Rosner introduce PPMx, adding covariate similarity to product-partition cohesion. This is direct lineage for data- or design-dependent partition priors. BayesBreak's contribution is a restricted ordered-contiguous factorization that makes segment cohesion and boundary hazard explicit and preserves exact normalization by dynamic programming. The source prevents claims that covariate-dependent or design-aware cohesion is new in general.


==> shared/bibliography/annotated_entries/olshen2004cbs.tex <==

\paragraph{\texttt{olshen2004cbs}: \citet{olshen2004cbs}.}
Olshen and coauthors introduce circular binary segmentation for array-based DNA copy-number analysis. CBS is a domain-standard comparator for the array-CGH case study. It operates on point-estimate segmentation rather than BayesBreak's posterior partition distribution. The archived CGH comparator computation is excluded from scientific comparison because a $43\times2215$ fitted array was flattened to 95,245 values while the BayesBreak boundaries remained on the 2,215-probe axis; that execution cannot support a scientific comparison.


==> shared/bibliography/annotated_entries/park2010gppm.tex <==

\paragraph{\texttt{park2010gppm}: \citet{park2010gppm}.}
Park and Dunson develop generalized product partition models, broadening the ways local partition factors can encode prior structure. BayesBreak uses the work to situate its ordered prior specification: only factors that can be assigned locally to admissible contiguous blocks and interior endpoints can enter the unchanged finite DP. The book's result is therefore a transparent specialization and implementation rule, not a general invention of product-partition priors.


==> shared/bibliography/annotated_entries/polson2013pg.tex <==

\paragraph{\texttt{polson2013pg}: \citet{polson2013pg}.}
Polson, Scott, and Windle introduce P\'olya--Gamma data augmentation for Bayesian logistic models, yielding conditional Gaussian structure. BayesBreak uses this identity as an established route for block-local logistic computation and diagnostics. The source does not imply that a mean-field or approximate BayesBreak block score has a uniform rate over all reachable blocks. Such a rate would require additional assumptions and proof; in this book the global theorem is explicitly conditional on a supplied local error certificate.


==> shared/bibliography/annotated_entries/punskaya2002bayesian.tex <==

\paragraph{\texttt{punskaya2002bayesian}: \citet{punskaya2002bayesian}.}
Punskaya and coauthors develop Bayesian curve fitting by MCMC with signal-segmentation applications. The paper supplies a sampling-based Bayesian alternative that can accommodate models outside BayesBreak's exact factorized regime. BayesBreak uses it to motivate posterior uncertainty while explaining why its own exact recursions require segment-local integrated scores. It is not used to justify the archived BayesBreak numerical values.


==> shared/bibliography/annotated_entries/quinlan2024jrpm.tex <==

\paragraph{\texttt{quinlan2024jrpm}: \citet{quinlan2024jrpm}.}
Quinlan, Page, and Castro develop joint random partition models that permit dependence among multiple partitions. This is richer than BayesBreak's exact common-boundary specialization. The source is used to state the tradeoff precisely: BayesBreak gains a simple exact DP by imposing a shared partition (or known groups), while JRPM targets flexible dependence across series. Broad claims about general multivariate partition inference are therefore excluded.


==> shared/bibliography/annotated_entries/rigaill2010pruned.tex <==

\paragraph{\texttt{rigaill2010pruned}: \citet{rigaill2010pruned}.}
Rigaill develops pruned dynamic programming for recovering best segmentations over a range of segment counts. The work belongs to the optimization/pruning lineage and informs possible efficiency comparisons. BayesBreak's current core deliberately preserves the unpruned exact posterior recursion, so the empirical slopes near 1.07 and 1.14 are reported only as finite-range observations and never as a change to the $O(k_{\max}n^2)$ worst-case complexity.


==> shared/bibliography/annotated_entries/rudin1992rof.tex <==
\paragraph{\texttt{rudin1992rof}: \citet{rudin1992rof}.}
Rudin, Osher, and Fatemi introduce total-variation regularization for edge-preserving reconstruction. The work is a mathematical ancestor of piecewise-constant penalization, not a Bayesian changepoint posterior method. BayesBreak uses this lineage to contextualize fused and total-variation baselines and to distinguish a penalized point estimator from a posterior distribution over partitions.


==> shared/bibliography/annotated_entries/ruggieri2014bcpvs.tex <==

\paragraph{\texttt{ruggieri2014bcpvs}: \citet{ruggieri2014bcpvs}.}
Ruggieri and Lawrence combine Bayesian changepoint inference with variable selection and apply the method to a paleoclimate proxy record. The work demonstrates that scientifically meaningful segmentation often couples regime changes with additional structural choices. BayesBreak cites it as an application and model-extension lineage while keeping variable selection outside the protected core. It informs future-work boundaries rather than a current contribution claim.


==> shared/bibliography/annotated_entries/scargle2013bayesianblocks.tex <==

\paragraph{\texttt{scargle2013bayesianblocks}: \citet{scargle2013bayesianblocks}.}
Scargle and coauthors develop Bayesian Blocks for optimal representations under arbitrary sampling modes, gaps, exposures, and several data modes. This is important prior art for irregularly sampled segmentation. BayesBreak therefore narrows its claim: likelihood exposure, segment cohesion, and boundary hazard are distinct modeling components, and ordered cohesion-plus-hazard factors can be consumed by the same DP. The source is closest work for irregular-design handling, not support for the earlier conflated Poisson-gap derivation.


==> shared/bibliography/annotated_entries/teicher1963identifiability.tex <==
\paragraph{\texttt{teicher1963identifiability}: \citet{teicher1963identifiability}.}
Teicher establishes classical identifiability results for finite mixtures under conditions on normalized component distributions. The reference is retained to mark a boundary of applicability. BayesBreak's current subject--template scores are positive partition scores rather than normalized subject-level component densities, so finite-mixture identifiability does not follow from Teicher's result. The book limits the established latent-template theory to monotonicity of the stated objective and records label permutations, duplicate templates, and collapsed solutions as failure modes.


==> shared/bibliography/annotated_entries/tibshirani2005fused.tex <==
\paragraph{\texttt{tibshirani2005fused}: \citet{tibshirani2005fused}.}
Tibshirani and coauthors formulate the fused lasso, combining sparsity and adjacent-difference penalties to estimate piecewise-constant structure. It is a natural point-estimation baseline for offline segmentation. BayesBreak differs through probabilistic integration over segment parameters and posterior inference over changepoint configurations; a fused-lasso tuning path is not equivalent to a prior on the number of segments. The source informs baseline selection and misspecification analysis.


==> shared/bibliography/annotated_entries/tierney1986laplace.tex <==
\paragraph{\texttt{tierney1986laplace}: \citet{tierney1986laplace}.}
Tierney and Kadane develop Laplace approximations for posterior moments and marginal posterior densities under regularity conditions that include a suitably regular, unimodal likelihood-times-prior integrand. BayesBreak cites this paper as a foundation for Laplace evaluation of a nonconjugate segment marginal likelihood. The source does not imply a uniform error bound over all candidate segments, nor does it establish a BayesBreak-specific convergence rate. Any use in BayesBreak therefore requires the segment objective, mode, curvature, and approximation error to be assessed over the admissible segment set; the partition-level error statements apply only after such a segment-level bound has been established.


==> shared/bibliography/annotated_entries/truong2020review.tex <==

\paragraph{\texttt{truong2020review}: \citet{truong2020review}.}
Truong, Oudre, and Vayatis provide a selective review and taxonomy of offline changepoint methods, including costs, search methods, and evaluation considerations. BayesBreak uses the review to organize baseline families and to prevent category errors between detection, segmentation, online monitoring, and posterior inference. It is a secondary synthesis rather than evidence for a BayesBreak theorem or result.


==> shared/bibliography/annotated_entries/yao1988biometrika.tex <==
\paragraph{\texttt{yao1988biometrika}: \citet{yao1988biometrika}.}
Yao studies estimation of the number of changepoints in an independent normal sequence using Schwarz's criterion and establishes weak consistency of the proposed estimator. This paper represents information-criterion selection of segment count. BayesBreak uses it as a contrast to assigning a prior to the number of segments, integrating over that number, and reporting its posterior distribution together with posterior changepoint summaries and a separate joint MAP partition. These procedures address related but nonidentical inferential targets.


==> shared/brand/colors.tex <==
% SAIM semantic color system - single source of truth.
% Load xcolor before inputting this file.

% Core brand colors derived from the supplied SAIM identity.
\definecolor{SAIMIndigo}{HTML}{32127A}
\definecolor{SAIMIndigoDark}{HTML}{1A0A40}
\definecolor{SAIMLavender}{HTML}{D6CFE4}
\definecolor{SAIMLavenderLight}{HTML}{F5F2FA}
\definecolor{SAIMInk}{HTML}{17131F}
\definecolor{SAIMDark}{HTML}{211934}
\definecolor{SAIMCoolGray}{HTML}{F4F2F8}
\definecolor{SAIMPanel}{HTML}{FAF9FC}
\definecolor{SAIMMuted}{HTML}{6F6879}
\definecolor{SAIMRule}{HTML}{D8D3E1}
\definecolor{SAIMRuleDark}{HTML}{978EA7}
\definecolor{SAIMBlue}{HTML}{2E5C8A}
\definecolor{SAIMBluePale}{HTML}{EAF2F8}
\definecolor{SAIMGreen}{HTML}{4A7A5C}
\definecolor{SAIMGreenPale}{HTML}{EAF3ED}
\definecolor{SAIMRed}{HTML}{A74455}
\definecolor{SAIMRedPale}{HTML}{F8EAEE}
\definecolor{SAIMAmber}{HTML}{9B6418}
\definecolor{SAIMAmberPale}{HTML}{FFF4DD}

% Semantic names shared by the paper, slides, lecture notes, book, and gallery.
% White remains the default page and component interior; lavender is reserved
% for selected emphasis, diagrams, and optional soft backgrounds.
\colorlet{Primary}{SAIMIndigo}
\colorlet{PrimaryDark}{SAIMIndigoDark}
\colorlet{PrimaryPale}{white}
\colorlet{PrimaryWash}{white}
\colorlet{Secondary}{SAIMBlue}
\colorlet{SecondaryPale}{SAIMBluePale}
\colorlet{Positive}{SAIMGreen}
\colorlet{PositivePale}{SAIMGreenPale}
\colorlet{Negative}{SAIMRed}
\colorlet{NegativePale}{SAIMRedPale}
\colorlet{Warning}{SAIMAmber}
\colorlet{WarningPale}{SAIMAmberPale}
\colorlet{Ink}{SAIMInk}
\colorlet{Muted}{SAIMMuted}
\colorlet{Rule}{SAIMRule}
\colorlet{RuleDark}{SAIMRuleDark}
\colorlet{CodeBackground}{SAIMCoolGray}
\colorlet{LightPanel}{SAIMPanel}

% Compatibility aliases retained from the supplied SAIM templates.
\colorlet{saimindigo}{Primary}
\colorlet{saimbg}{SAIMLavender}
\colorlet{saimfg}{Ink}
\colorlet{saimdark}{SAIMDark}
\colorlet{saimgray}{SAIMCoolGray}
\colorlet{saimblue}{Secondary}
\colorlet{saimgreen}{Positive}
\colorlet{saimlight}{SAIMLavenderLight}
\colorlet{lightblue}{SecondaryPale}
\colorlet{metablue}{Secondary}
\colorlet{metafg}{Ink}
\colorlet{metabg}{LightPanel}


==> shared/brand/typography.tex <==
% SAIM Computer Modern Sans typography system - single source of truth.
% This reproduces the font system used by the reference Beamer deck:
% Computer Modern Sans for text, Computer Modern Typewriter for code, and the
% classic Computer Modern / AMS families for mathematics.
%
% The exact reference rendering is a pdfLaTeX system. No uploaded font files
% are required; all fonts ship with a standard TeX distribution.
\RequirePackage{fix-cm}
\RequirePackage[utf8]{inputenc}
\RequirePackage{textcomp}
\RequirePackage[protrusion=true,expansion=true]{microtype}
\RequirePackage{setspace}

% Use classic Computer Modern Sans everywhere ordinary text is requested.
% Mapping both Roman and Sans roles to cmss also converts legacy explicit
% \rmfamily calls in the template without creating a second visual family.
\renewcommand{\rmdefault}{cmss}
\renewcommand{\sfdefault}{cmss}
\renewcommand{\ttdefault}{cmtt}
\renewcommand{\familydefault}{\sfdefault}

% Computer Modern Sans provides a slanted face rather than a separate italic
% face. Route ordinary italic requests to that native slanted design so prose,
% citations, and code comments remain inside the reference font family.
\DeclareFontShape{OT1}{cmss}{m}{it}{<->ssub*cmss/m/sl}{}
\DeclareFontShape{OT1}{cmss}{bx}{it}{<->ssub*cmss/bx/n}{}
\normalfont

% Semantic font roles. All prose and display text share Computer Modern Sans;
% Mono marks technical literals. Mathematics remains the standard Computer
% Modern math system loaded by LaTeX and the AMS packages.
\providecommand{\SAIMBodyFont}{\sffamily}
\providecommand{\SAIMHeadingFont}{\sffamily\bfseries}
\providecommand{\SAIMCoverTitleFont}{\sffamily\bfseries}
\providecommand{\SAIMCoverSubtitleFont}{\sffamily}
\providecommand{\SAIMNavigationFont}{\sffamily\bfseries}
\providecommand{\SAIMMetaFont}{\sffamily}
\providecommand{\SAIMCodeFont}{\ttfamily}

% Compatibility aliases used by the front-matter implementations.
\providecommand{\SAIMFrontFont}{\sffamily}
\providecommand{\SAIMFrontTitleFont}{\SAIMCoverTitleFont}
\providecommand{\SAIMFrontMetaFont}{\SAIMMetaFont}
\providecommand{\SAIMFrontRagged}{\raggedright\hyphenpenalty=10000\exhyphenpenalty=10000}


==> shared/components/bayesbreak-book-compat.tex <==
% Book-specific macro compatibility. Deliberately omits definitions already
% owned by shared/components/bayesbreak.tex.
\providecommand{\ProofStep}[1]{\par\smallskip\noindent\textbf{#1}\quad}
\providecommand{\1}{\mathbbm{1}}
\providecommand{\eps}{\varepsilon}
\providecommand{\figref}[1]{figure~\ref{#1}}
\providecommand{\Figref}[1]{Figure~\ref{#1}}
\providecommand{\secref}[1]{section~\ref{#1}}
\providecommand{\Secref}[1]{Section~\ref{#1}}
\providecommand{\algref}[1]{algorithm~\ref{#1}}
\providecommand{\Algref}[1]{Algorithm~\ref{#1}}
\providecommand{\Eqref}[1]{Equation~\ref{#1}}
\providecommand{\ceil}[1]{\lceil #1\rceil}
\providecommand{\floor}[1]{\lfloor #1\rfloor}
\newtheorem{example}[theorem]{Example}
\newtheorem{targettheorem}[theorem]{Target theorem}
\newtheorem{proofobligation}[theorem]{Proof obligation}

\providecommand{\EstablishedTag}{\SAIMEvidenceTag{Positive}{PositivePale}{Established}}
\providecommand{\ExactDerivedTag}{\SAIMEvidenceTag{Secondary}{SecondaryPale}{Exact derivation}}
\providecommand{\RealResultTag}{\SAIMEvidenceTag{Positive}{PositivePale}{Real result}}
\providecommand{\PartialTag}{\SAIMEvidenceTag{Warning}{WarningPale}{Partial}}
\providecommand{\TargetTag}{\SAIMEvidenceTag{RuleDark}{LightPanel}{Target}}
\providecommand{\ExcludedTag}{\SAIMEvidenceTag{PrimaryDark}{PrimaryWash}{Excluded}}
\providecommand{\ConditionalTag}{\SAIMEvidenceTag{Warning}{WarningPale}{Conditional}}
\providecommand{\ExternalVerifiedTag}{\SAIMEvidenceTag{Secondary}{SecondaryPale}{Verified external}}

\newtcolorbox{statusbox}[1][Result status]{
 enhanced,breakable,colback=PrimaryWash,colframe=Primary,boxrule=0.6pt,arc=2pt,
 left=10pt,right=10pt,top=8pt,bottom=8pt,before skip=9pt,after skip=10pt,
 title={\rmfamily\bfseries\fontsize{7.1}{8.4}\selectfont\color{PrimaryDark}\MakeUppercase{#1}},
 attach title to upper={\par\vspace{5pt}}}
\providecommand{\taskid}[1]{\texttt{#1}}
\providecommand{\Real}{\mathbb{R}}
\providecommand{\bbone}{\mathbbm{1}}
\providecommand{\NA}{\textsc{na}}
\providecommand{\pluseq}{\mathrel{+}=}
\providecommand{\code}[1]{\texttt{#1}}
\newenvironment{takeawaybox}{\begin{keyidea}}{\end{keyidea}}

% tikz-bayesnet 0.1 terminates \foreach blocks with standalone semicolon
% tokens, which pdfTeX reports as missing characters in nullfont. These
% equivalent local definitions retain the drawing paths but remove those
% non-drawing tokens so clean builds have no false missing-glyph warnings.
\renewcommand{\edge}[3][]{%
  \foreach \x in {#2}{%
    \foreach \y in {#3}{%
      \draw[->,#1] (\x) -- (\y);%
    }%
  }%
}
\renewcommand{\plate}[4][]{%
  \node[wrap=#3] (#2-wrap) {};%
  \node[plate caption=#2-wrap] (#2-caption) {#4};%
  \node[plate=(#2-wrap)(#2-caption),#1] (#2) {};%
}


==> shared/components/bayesbreak-compat.tex <==

% Compatibility and project vocabulary for the reconstructed BayesBreak source.
\newcommand{\ProofStep}[1]{\par\smallskip\noindent\textbf{#1}\quad}
\providecommand{\Var}{\operatorname{Var}}
\providecommand{\Cov}{\operatorname{Cov}}
\providecommand{\KL}{D_{\mathrm{KL}}}
\providecommand{\softmax}{\operatorname{softmax}}
\providecommand{\logsumexp}{\operatorname{logsumexp}}
\providecommand{\1}{\mathbbm{1}}
\providecommand{\eps}{\varepsilon}
\providecommand{\figref}[1]{figure~\ref{#1}}
\providecommand{\Figref}[1]{Figure~\ref{#1}}
\providecommand{\secref}[1]{section~\ref{#1}}
\providecommand{\Secref}[1]{Section~\ref{#1}}
\providecommand{\algref}[1]{algorithm~\ref{#1}}
\providecommand{\Algref}[1]{Algorithm~\ref{#1}}
\providecommand{\Eqref}[1]{Equation~\ref{#1}}
\providecommand{\ceil}[1]{\lceil #1\rceil}
\providecommand{\floor}[1]{\lfloor #1\rfloor}
\newtheorem{example}[theorem]{Example}
\newtheorem{targettheorem}[theorem]{Target theorem}
\newtheorem{proofobligation}[theorem]{Proof obligation}

\newcommand{\EstablishedTag}{\CSEvidenceTag{Positive}{PositivePale}{Established}}
\newcommand{\ExactDerivedTag}{\CSEvidenceTag{Secondary}{SecondaryPale}{Exact derivation}}
\newcommand{\RealResultTag}{\CSEvidenceTag{Positive}{PositivePale}{Real result}}
\newcommand{\PartialTag}{\CSEvidenceTag{Warning}{WarningPale}{Partial}}
\newcommand{\TargetTag}{\CSEvidenceTag{RuleDark}{LightPanel}{Target}}
\newcommand{\ExcludedTag}{\CSEvidenceTag{PrimaryDark}{PrimaryWash}{Excluded}}
\newcommand{\ConditionalTag}{\CSEvidenceTag{Warning}{WarningPale}{Conditional}}
\newcommand{\ExternalVerifiedTag}{\CSEvidenceTag{Secondary}{SecondaryPale}{Verified external}}

\newtcolorbox{statusbox}[1][Evidence status]{
 enhanced,breakable,colback=PrimaryWash,colframe=Primary,boxrule=0.6pt,arc=2pt,
 left=10pt,right=10pt,top=8pt,bottom=8pt,before skip=9pt,after skip=10pt,
 title={\rmfamily\bfseries\fontsize{7.1}{8.4}\selectfont\color{PrimaryDark}\MakeUppercase{#1}},
 attach title to upper={\par\vspace{5pt}}}
\newcommand{\taskid}[1]{\texttt{#1}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\bbone}{\mathbbm{1}}
\newcommand{\NA}{\textsc{na}}
\newcommand{\pluseq}{\mathrel{+}=}
\newcommand{\code}[1]{\texttt{#1}}
\newenvironment{takeawaybox}{\begin{keyidea}}{\end{keyidea}}


==> shared/components/bayesbreak.tex <==
% BayesBreak-specific mathematical, result-status, and authoring layer.
\RequirePackage{bm}
\RequirePackage{longtable}
\RequirePackage{makecell}
\RequirePackage{pdflscape}
\RequirePackage{adjustbox}
\RequirePackage{microtype}
\RequirePackage{xspace}
\RequirePackage{etoolbox}
\RequirePackage{url}
\RequirePackage{enumitem}
\RequirePackage{csquotes}
\graphicspath{{figures/}{shared/figures/tikz/}}
\newcommand{\BayesBreak}{\textsc{BayesBreak}\xspace}
\newcommand{\claimid}[1]{\texttt{#1}}
\newcommand{\resultid}[1]{\texttt{#1}}
\newcommand{\experimentid}[1]{\texttt{#1}}
\newcommand{\codeid}[1]{\texttt{#1}}
\newcommand{\diagramid}[1]{\texttt{#1}}
\newcommand{\criterionid}[1]{\texttt{#1}}
\newcommand{\Rset}{\mathbb{R}}
\newcommand{\Nset}{\mathbb{N}}
\newcommand{\Ind}{\mathbbm{1}}
\newcommand{\trans}{\mathsf{T}}
\newcommand{\given}{\,\middle|\,}
\newcommand{\dd}{\,\mathrm{d}}
\newcommand{\KL}{\operatorname{KL}}
\newcommand{\TV}{\operatorname{TV}}
\newcommand{\logsumexp}{\operatorname{LSE}}
\DeclareMathOperator{\softmax}{softmax}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\BetaFn}{B}
\newcommand{\statuspill}[2]{\begingroup\setlength{\fboxsep}{3pt}\colorbox{#1}{\textcolor{white}{\sffamily\bfseries\scriptsize #2}}\endgroup}
\newcommand{\Established}{\statuspill{Positive}{ESTABLISHED}}
\newcommand{\ExactDerived}{\statuspill{Primary}{EXACTLY DERIVED}}
\newcommand{\RealEvidence}{\statuspill{Secondary}{EXECUTED RESULT}}
\newcommand{\PartiallySupported}{\statuspill{Warning}{PARTIAL}}
\newcommand{\Planned}{\statuspill{Muted}{PLANNED}}
\newcommand{\ExcludedResult}{\statuspill{Negative}{EXCLUDED}}
\newcommand{\ProofObligation}{\statuspill{Warning}{PROOF OBLIGATION}}
\newtcolorbox{exclusionbox}[1][Excluded computation]{enhanced,breakable,colback=NegativePale,colframe=Negative,boxrule=.7pt,arc=2pt,left=10pt,right=10pt,top=8pt,bottom=8pt,before skip=9pt,after skip=9pt,title={\rmfamily\bfseries\fontsize{7.1}{8.4}\selectfont\color{Negative}\textls[125]{\MakeUppercase{#1}}},attach title to upper={\par\vspace{5pt}}}
\newtcolorbox{targetbox}[1][Target theorem / proof obligation]{enhanced,breakable,colback=WarningPale,colframe=Warning,boxrule=.7pt,arc=2pt,left=10pt,right=10pt,top=8pt,bottom=8pt,before skip=9pt,after skip=9pt,title={\rmfamily\bfseries\fontsize{7.1}{8.4}\selectfont\color{Warning}\textls[120]{\MakeUppercase{#1}}},attach title to upper={\par\vspace{5pt}}}
\newtcolorbox{cautionbox}[1][Failure state]{enhanced,breakable,colback=WarningPale,colframe=Warning,boxrule=.7pt,arc=2pt,left=10pt,right=10pt,top=8pt,bottom=8pt,before skip=9pt,after skip=9pt,title={\rmfamily\bfseries\fontsize{7.1}{8.4}\selectfont\color{Warning}\textls[120]{\MakeUppercase{#1}}},attach title to upper={\par\vspace{5pt}}}
\newtcolorbox{specificationbox}[1][Interface specification]{enhanced,breakable,colback=PrimaryWash,colframe=Primary,boxrule=.65pt,arc=2pt,left=10pt,right=10pt,top=8pt,bottom=8pt,before skip=9pt,after skip=9pt,title={\rmfamily\bfseries\fontsize{7.1}{8.4}\selectfont\color{PrimaryDark}\textls[125]{\MakeUppercase{#1}}},attach title to upper={\par\vspace{5pt}}}
\newcommand{\evidencekey}{\begin{center}\begin{tabularx}{\textwidth}{@{}lX@{}}\toprule\textbf{Marker} & \textbf{Meaning in this book}\\\midrule\Established & Complete derivation or theorem with an immediate proof under stated assumptions.\\\ExactDerived & Algebraic formula or identity derived exactly but not promoted to a priority claim.\\\RealEvidence & A populated value from an executed archived computation.\\\PartiallySupported & The computation is real or the statement is valid only under a restricted interpretation.\\\Planned & Protocol or artifact is specified but not executed or not populated.\\\ExcludedResult & The computation is retained in the record but excluded from the stated analysis because its model, axis, family, or support is invalid.\\\bottomrule\end{tabularx}\end{center}}
\newcommand{\sourceanchor}[1]{\par\smallskip{\footnotesize\color{Muted}\textbf{Source:} \texttt{#1}}}
\newcommand{\evidencestatus}[2]{\par\smallskip{\footnotesize\textbf{Result status:} #1\quad #2}}
\newcommand{\resultnote}[3]{\begin{evidencebox}[#1]\resultid{#2}. #3\end{evidencebox}}
\newenvironment{bbalgorithm}[1]{\begin{tcolorbox}[enhanced,breakable,colback=white,colframe=Primary,boxrule=.7pt,arc=2pt,left=10pt,right=10pt,top=9pt,bottom=9pt,before skip=10pt,after skip=10pt,title={\rmfamily\bfseries\color{white}#1},colbacktitle=Primary]}{\end{tcolorbox}}
\newcommand{\tighttable}{\small\renewcommand{\arraystretch}{1.15}\setlength{\tabcolsep}{4.2pt}}

% Stable authoring helpers.
\newcommand{\bbchapterid}[1]{\marginnote{\RaggedRight\scriptsize\ttfamily\color{Muted}#1}}
\newcommand{\bbassetid}[1]{\texttt{#1}}
\newcommand{\bbterm}[1]{\textbf{#1}}
\newcommand{\bbfig}[4][\textwidth]{%
  \begin{figure}[tbp]
  \centering
  \resizebox{#1}{!}{\input{#2}}
  \caption{#3}\label{#4}
  \end{figure}}
\newcommand{\bbresultfig}[4][0.96\textwidth]{%
  \begin{figure}[tbp]
  \centering
  \includegraphics[width=#1]{#2}
  \caption{#3}\label{#4}
  \end{figure}}
\newcommand{\bbstatusline}[2]{\par\smallskip{\footnotesize\textbf{Status:} #1\quad #2}\par\smallskip}
\newcommand{\bbsource}[1]{{\footnotesize\color{Muted}\textbf{Source:} \texttt{#1}}}
\newcommand{\bbna}{\texttt{NA}}
\newcommand{\bbtodo}[1]{\textcolor{Warning}{\textbf{PLANNED: #1}}}
\newenvironment{claimbox}[1][Claim statement]{\begin{specificationbox}[#1]}{\end{specificationbox}}


==> shared/components/boxes.tex <==
% Shared tcolorbox vocabulary.
% Load tcolorbox with the `most` library before inputting this file.
\tcbset{
  saim/base/.style={
    enhanced,
    breakable,
    boxrule=0pt,
    arc=1.5pt,
    outer arc=1.5pt,
    left=8pt,
    right=8pt,
    top=7pt,
    bottom=7pt,
    before skip=8pt,
    after skip=8pt,
    fonttitle=\rmfamily\bfseries,
    coltitle=Ink,
    attach title to upper={\par\vspace{2pt}},
  },
  saim/primary/.style={
    saim/base,
    colback=PrimaryWash,
    borderline west={2.4pt}{0pt}{Primary},
    colframe=Primary,
  },
  saim/blue/.style={
    saim/base,
    colback=SecondaryPale,
    borderline west={2.4pt}{0pt}{Secondary},
    colframe=Secondary,
  },
  saim/green/.style={
    saim/base,
    colback=PositivePale,
    borderline west={2.4pt}{0pt}{Positive},
    colframe=Positive,
  },
  saim/amber/.style={
    saim/base,
    colback=WarningPale,
    borderline west={2.4pt}{0pt}{Warning},
    colframe=Warning,
  },
  saim/neutral/.style={
    saim/base,
    colback=LightPanel,
    borderline west={2.4pt}{0pt}{RuleDark},
    colframe=Rule,
  },
  saim/outline/.style={
    enhanced,
    breakable,
    colback=white,
    colframe=Rule,
    boxrule=0.55pt,
    arc=2pt,
    outer arc=2pt,
    left=8pt,
    right=8pt,
    top=7pt,
    bottom=7pt,
    before skip=8pt,
    after skip=8pt,
    fonttitle=\rmfamily\bfseries,
    coltitle=Ink,
  },
}


==> shared/components/evidence.tex <==
% Compact evidence-status labels usable in paper, slides, and book.
% Requires xcolor; no other package dependency.
\newcommand{\SAIMEvidenceTag}[3]{%
  \begingroup
  \setlength{\fboxsep}{2.6pt}%
  \setlength{\fboxrule}{0.45pt}%
  \raisebox{0.2ex}{\fcolorbox{#1}{#2}{%
    \textcolor{#1}{\sffamily\bfseries\fontsize{6.8}{8}\selectfont\textls[65]{\strut\MakeUppercase{#3}}}}}%
  \endgroup}
\newcommand{\MeasuredTag}{\SAIMEvidenceTag{Positive}{PositivePale}{Measured}}
\newcommand{\ReproducedTag}{\SAIMEvidenceTag{Secondary}{SecondaryPale}{Reproduced}}
\newcommand{\SyntheticTag}{\SAIMEvidenceTag{Warning}{WarningPale}{Synthetic}}
\newcommand{\PlannedTag}{\SAIMEvidenceTag{RuleDark}{LightPanel}{Planned}}
\newcommand{\IllustrativeTag}{\SAIMEvidenceTag{PrimaryDark}{PrimaryWash}{Illustrative}}
\newcommand{\ExternalTag}{\SAIMEvidenceTag{Secondary}{SecondaryPale}{External}}


==> shared/components/frontmatter.tex <==
% Shared front-page typography roles.
% Computer Modern Sans is used consistently for title hierarchy, metadata,
% navigation, and prose, matching the reference Beamer deck.
\providecommand{\SAIMFrontFont}{\sffamily}
\providecommand{\SAIMFrontTitleFont}{\SAIMCoverTitleFont}
\providecommand{\SAIMFrontMetaFont}{\SAIMMetaFont}
\providecommand{\SAIMFrontRagged}{\raggedright\hyphenpenalty=10000\exhyphenpenalty=10000}


==> shared/components/listings.tex <==
% Shared code-listing styles. Load listings before inputting this file.
\lstdefinestyle{python}{
  language=Python,
  basicstyle=\ttfamily\small\color{Ink},
  keywordstyle=\color{PrimaryDark}\bfseries,
  stringstyle=\color{Positive},
  commentstyle=\color{Muted}\itshape,
  numberstyle=\scriptsize\color{RuleDark},
  numbers=left,
  numbersep=9pt,
  backgroundcolor=\color{CodeBackground},
  frame=leftline,
  rulecolor=\color{Primary},
  framerule=1.4pt,
  breaklines=true,
  showstringspaces=false,
  keepspaces=true,
  columns=fullflexible,
  xleftmargin=12pt,
  framexleftmargin=4pt,
  aboveskip=9pt,
  belowskip=9pt,
  captionpos=t,
}
\lstdefinestyle{console}{
  basicstyle=\ttfamily\small\color{Ink},
  backgroundcolor=\color{LightPanel},
  frame=leftline,
  rulecolor=\color{Secondary},
  framerule=1.4pt,
  breaklines=true,
  columns=fullflexible,
  xleftmargin=12pt,
  framexleftmargin=4pt,
  aboveskip=9pt,
  belowskip=9pt,
  captionpos=t,
}


==> shared/components/table-columns.tex <==
% Shared table vocabulary. Load array and tabularx first.
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}
\newcolumntype{Z}{>{\centering\arraybackslash}X}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcommand{\CSTableHead}[1]{{\rmfamily\bfseries\color{Ink}#1}}
\newcommand{\CSBest}[1]{{\bfseries\color{Positive}#1}}
\newcommand{\CSMutedCell}[1]{{\color{Muted}#1}}


==> shared/figures/defs/fig3_boundary_calibration.tex <==
\begin{figure}[!htbp]
  \centering
  \includegraphics[width=0.78\textwidth,keepaspectratio]{figures/fig3_boundary_calibration.pdf}
  \caption{Calibration of marginal boundary posterior probabilities under synthetic
  Gaussian data (E01, $n=256$, 100 sequences per stratum). The dashed diagonal
  denotes perfect calibration; the curve is the empirical frequency within
  equal-mass bins of predicted posterior boundary probability. Mid-probability
  bins show the most variability because boundary events are intrinsically rare
  per sequence, but the ordering of confidence levels is consistent with
  calibration: bins assigned higher posterior probability correspond to
  higher empirical frequency.}
  \label{fig:calibration}
\end{figure}


==> shared/figures/defs/fig5_runtime_scaling.tex <==
\begin{figure}[!htbp]
  \centering
  \includegraphics[width=0.92\textwidth,height=0.67\textheight,keepaspectratio]{figures/fig5_runtime_scaling.png}
  \caption{Gaussian runtime measurements. Points are means over five repetitions
    and error bars are one standard deviation. Dashed references show
    quadratic-in-$n$ and linear-in-$k_{\max}$ guides, not fitted complexity claims.}
  \label{fig:runtime-result-paper}
\end{figure}


==> shared/figures/defs/fig8_spx.tex <==
\begin{figure}[!htbp]
  \centering
  \includegraphics[width=0.90\textwidth,height=0.43\textheight,keepaspectratio]{figures/fig8_spx.png}
  \caption{S\&P 500 volatility fit after stride-four preprocessing. Red markers are fitted
    boundaries, not independently annotated macroeconomic events.}
  \label{fig:spx-paper}
\end{figure}


==> shared/figures/defs/fig_cgh_probe_agreement.tex <==
\begin{figure}[!htbp]
  \centering
  \includegraphics[width=0.83\textwidth,height=0.41\textheight,keepaspectratio]{figures/fig_cgh_probe_agreement.png}
  \caption{Probe-aligned array-CGH comparison. Top: boundary locations on the shared probe axis.
    Bottom: $F_1@3$ and exact Jaccard agreement with the model-derived BayesBreak MAP.}
  \label{fig:cgh-agreement-corrected-paper}
\end{figure}


==> shared/figures/medium-calibration.tex <==
% Three-medium design comparison; no surrounding figure environment.
\newcommand{\CSMediumCalibrationDiagram}{%
\begin{tikzpicture}[
  every node/.style={font=\rmfamily},
  card/.style={draw=Rule,fill=white,rounded corners=2pt,
    minimum width=39mm,minimum height=32mm,text width=34mm,
    align=left,inner sep=4mm,line width=0.55pt},
]
  \node[card] (paper) {\textcolor{Primary}{\scriptsize\bfseries PAPER}\\[3pt]
    \textbf{Editorial density}\\[2pt]
    \scriptsize Restrained branding, compact evidence, precise captions, and
    publication-friendly typography.};
  \node[card,right=6mm of paper] (slides) {\textcolor{Primary}{\scriptsize\bfseries SLIDES}\\[3pt]
    \textbf{Claim-led pacing}\\[2pt]
    \scriptsize Solid-orange bookends, editorial section dividers, and one
    visual argument per frame.};
  \node[card,right=6mm of slides] (book) {\textcolor{Primary}{\scriptsize\bfseries BOOK}\\[3pt]
    \textbf{Pedagogical depth}\\[2pt]
    \scriptsize Chapter promises, margin notes, worked examples, exercises,
    and reproducible implementation detail.};
\end{tikzpicture}%
}


==> shared/figures/system-overview.tex <==
\begin{figure}[htbp]
\centering
\begin{tikzpicture}[node distance=8mm and 6mm]
  \node[secondarybox,minimum width=28mm] (data) {Inputs\\[-1pt]\scriptsize data, requirements};
  \node[primarybox,minimum width=28mm,right=of data] (method) {Method\\[-1pt]\scriptsize model, objective};
  \node[neutralbox,minimum width=28mm,right=of method] (impl) {Implementation\\[-1pt]\scriptsize training, serving};
  \node[successbox,minimum width=28mm,right=of impl] (eval) {Evidence\\[-1pt]\scriptsize quality, cost, risk};
  \draw[arrSecondary] (data) -- (method);
  \draw[arrPrimary] (method) -- (impl);
  \draw[arr] (impl) -- (eval);
  \draw[arr,dashed] (eval.south) -- ++(0,-8mm) -|
    node[pos=0.52,below=1mm,font=\scriptsize\rmfamily,text=Muted]
      {diagnose and revise} (method.south);
\end{tikzpicture}
\caption{Canonical book workflow. The narrative moves left to right, while
evaluation feeds back into method revision. Replace the labels with the actual
components of the book.}
\label{fig:system-overview}
\end{figure}


==> shared/figures/tikz/experiments/claim_experiment_result_map.tex <==
\begin{tikzpicture}[node distance=7mm and 8mm]
\node[primarybox,text width=23mm] (claim) {Statistical claim};
\node[secondarybox,right=of claim,text width=28mm] (hyp) {Hypothesis and competing explanation};
\node[primarybox,right=of hyp,text width=25mm] (protocol) {Data-generating process or dataset, estimand, and metric};
\node[primarybox,right=of protocol,text width=24mm] (run) {Executed calculation and recorded output};
\node[successbox,right=of run,text width=27mm] (decision) {Permitted scientific interpretation};
\draw[arrPrimary] (claim)--(hyp);
\draw[arrPrimary] (hyp)--(protocol);
\draw[arrPrimary] (protocol)--(run);
\draw[arrPrimary] (run)--(decision);
\node[draw=Warning,fill=WarningPale,rounded corners,below=9mm of run,text width=32mm,align=center] (excluded) {Exclude when the observation model, coordinate axis, reference, or metric is incompatible};
\draw[arr,draw=Warning] (run)--(excluded);
\end{tikzpicture}


==> shared/figures/tikz/models/executive_shared_boundary.tex <==
\begin{tikzpicture}[node distance=7mm and 8mm]
\node[neutralbox,text width=28mm] (part) {Common ordered partition\\$\tau=(t_0,\ldots,t_k)$};
\node[secondarybox,below left=9mm and 5mm of part,text width=25mm] (s1) {Sequence 1\\segment scores $M^{(1)}_{ij}$};
\node[secondarybox,below=9mm of part,text width=25mm] (s2) {Sequence $s$\\segment scores $M^{(s)}_{ij}$};
\node[secondarybox,below right=9mm and 5mm of part,text width=25mm] (sS) {Sequence $S$\\segment scores $M^{(S)}_{ij}$};
\node[primarybox,below=13mm of s2,text width=40mm] (pool) {Pooled segment score\\$\log M^{\rm shared}_{ij}=\sum_{s=1}^{S}\log M^{(s)}_{ij}$};
\draw[arrPrimary] (part)--(s1);
\draw[arrPrimary] (part)--(s2);
\draw[arrPrimary] (part)--(sS);
\draw[arrSecondary] (s1)--(pool);
\draw[arrSecondary] (s2)--(pool);
\draw[arrSecondary] (sS)--(pool);
\end{tikzpicture}


==> shared/figures/tikz/models/latent_group_templates.tex <==
\begin{tikzpicture}[node distance=8mm and 9mm]
\node[secondarybox,text width=31mm] (scores) {Sequence-specific template scores\\$S_s(\tau_g)>0$};
\node[primarybox,right=of scores,text width=29mm] (resp) {Auxiliary allocation weights\\$r_{sg}$};
\node[primarybox,right=of resp,text width=32mm] (update) {Alternating updates\\$\pi_g$ and $\tau_g$};
\node[successbox,right=of update,text width=31mm] (obj) {$\mathcal F=\sum_s\log\sum_g\pi_gS_s(\tau_g)$};
\draw[arrPrimary] (scores)--(resp);
\draw[arrPrimary] (resp)--(update);
\draw[arrPrimary] (update)--(obj);
\draw[arrSecondary] (obj.north) |- ++(0,7mm) -| node[pos=0.52,above,font=\scriptsize]{next iteration} (scores.north);
\node[neutralbox,below=10mm of resp,text width=101mm] {The updates maximize a Jensen minorizer of the stated finite latent-group criterion. The criterion is not interpreted as a normalized finite-mixture likelihood.};
\end{tikzpicture}


==> shared/figures/tikz/roadmaps/executive_implementation_sequence.tex <==
\begin{tikzpicture}[node distance=6mm and 7mm]
\node[successbox,text width=25mm] (fixed) {Author-fixed title, statistical narrative, and proofs};
\node[neutralbox,right=of fixed,text width=25mm] (prior) {S1: prior factors and exact-DP integration};
\node[neutralbox,right=of prior,text width=25mm] (latent) {S2: latent-group objective and stable pooling};
\node[neutralbox,right=of latent,text width=25mm] (pred) {S3: prediction, metrics, and comparator schemas};
\draw[arrPrimary] (fixed)--(prior);
\draw[arrPrimary] (prior)--(latent);
\draw[arrPrimary] (latent)--(pred);

\node[neutralbox,below=11mm of prior,text width=25mm] (tests) {S4: pinned test completion and profiling};
\node[neutralbox,right=of tests,text width=25mm] (rerun) {S5: corrected CGH and methylation runs};
\node[neutralbox,right=of rerun,text width=25mm] (expand) {S6: repeated calibration, robustness, and scaling};
\node[primarybox,right=of expand,text width=25mm] (release) {S7: independent review and research release};
\draw[arrPrimary] (pred.south) |- (tests.east);
\draw[arrPrimary] (tests)--(rerun);
\draw[arrPrimary] (rerun)--(expand);
\draw[arrPrimary] (expand)--(release);

\node[draw=Rule,dashed,rounded corners,fit=(prior)(latent)(pred)(tests)(rerun)(expand),inner sep=3.5mm,label=below:{\scriptsize implementation and validation still required}] {};
\end{tikzpicture}


==> shared/figures/tikz/roadmaps/executive_release_decisions.tex <==
\begin{tikzpicture}[node distance=7mm and 16mm]
\node[primarybox,text width=42mm] (start) {Implementation corrections S1--S4 completed, or affected claims narrowed};
\node[draw=Warning,fill=WarningPale,diamond,aspect=2.35,below=9mm of start,align=center,font=\scriptsize,text width=36mm] (q1) {Tests and numerical invariants satisfy the pre-specified criteria?};
\node[primarybox,below=9mm of q1,text width=42mm] (rerun) {Produce corrected runs with new result IDs and parent links};
\node[draw=Warning,fill=WarningPale,diamond,aspect=2.35,below=9mm of rerun,align=center,font=\scriptsize,text width=36mm] (q2) {Coordinates, observation family, metrics, and provenance valid?};
\node[primarybox,below=9mm of q2,text width=42mm] (review) {Independent statistical, numerical, and source review};
\node[draw=Warning,fill=WarningPale,diamond,aspect=2.35,below=9mm of review,align=center,font=\scriptsize,text width=36mm] (q3) {Claims match complete proofs and executed results?};
\node[successbox,below=9mm of q3,text width=42mm] (release) {Release book, papers, coding handoff, and result records};
\node[neutralbox,right=25mm of q2,text width=39mm] (correct) {Stop, correct the implementation, rerun, or narrow the affected claim};

\draw[arrPrimary] (start)--(q1);
\draw[arrPrimary] (q1)--node[right,font=\scriptsize]{yes}(rerun);
\draw[arrPrimary] (rerun)--(q2);
\draw[arrPrimary] (q2)--node[right,font=\scriptsize]{yes}(review);
\draw[arrPrimary] (review)--(q3);
\draw[arrPrimary] (q3)--node[right,font=\scriptsize]{yes}(release);
\draw[arr,draw=Warning] (q1.east) -| node[pos=0.25,above,font=\scriptsize]{no}(correct.north);
\draw[arr,draw=Warning] (q2.east) -- node[above,font=\scriptsize]{no}(correct.west);
\draw[arr,draw=Warning] (q3.east) -| node[pos=0.25,below,font=\scriptsize]{no}(correct.south);
\draw[arr,draw=Warning,dashed] (correct.north) |- (start.east);
\end{tikzpicture}


==> shared/figures/tikz/theory/segment_error_propagation.tex <==
\begin{tikzpicture}[node distance=7mm and 8mm]
\node[secondarybox,text width=33mm] (ref) {Reference and approximate log segment marginal likelihoods};
\node[primarybox,right=of ref,text width=29mm] (eps) {$|\widehat\ell_{ij}-\ell_{ij}|\le\varepsilon$ for every admissible segment};
\node[primarybox,right=of eps,text width=31mm] (part) {$k$-segment partition log-weight error at most $k\varepsilon$};
\node[successbox,right=of part,text width=33mm] (global) {Bounds for marginal likelihoods, posterior odds, and modal changepoints};
\draw[arrPrimary] (ref)--(eps);
\draw[arrPrimary] (eps)--(part);
\draw[arrPrimary] (part)--(global);
\node[below=5mm of part,font=\scriptsize,text width=66mm,align=center] {The implication is conditional: the numerical method must establish the segmentwise bound under its own assumptions.};
\end{tikzpicture}


==> shared/figures/tikz/theory/theorem_dependency_map.tex <==

\begin{tikzpicture}[node distance=8mm and 10mm]
\node[successbox,text width=28mm] (block) {Block integration\\established};
\node[successbox,right=of block,text width=28mm] (dp) {Sum-product identities\\established};
\node[successbox,right=of dp,text width=28mm] (map) {Max-sum correctness\\established};
\node[secondarybox,below=of dp,text width=28mm] (prior) {Cohesion + hazard\\repaired};
\node[successbox,below=of map,text width=28mm] (shared) {Finite-candidate consistency\\established under conditions};
\node[secondarybox,below=of block,text width=28mm] (score) {Score-template monotonicity\\repaired};
\node[primarybox,below=of prior,text width=28mm] (approx) {Segment-score error propagation\\conditional};
\draw[arrPrimary] (block)--(dp);\draw[arrPrimary] (dp)--(map);
\draw[arrPrimary] (prior)--(dp);\draw[arrPrimary] (block)--(shared);\draw[arrPrimary] (dp)--(shared);
\draw[arrPrimary] (block)--(score);\draw[arrPrimary] (block)--(approx);\draw[arrPrimary] (dp)--(approx);
\end{tikzpicture}


==> shared/figures/tikz/workflows/posterior_prediction_workflow.tex <==
\begin{tikzpicture}[node distance=7mm and 8mm]
\node[secondarybox,text width=29mm] (post) {Posterior distribution for each fitted segment};
\node[primarybox,right=of post,text width=29mm] (cond) {Condition on a MAP partition or average over partitions};
\node[primarybox,right=of cond,text width=29mm] (coord) {Check prediction coordinate against fitted support};
\node[successbox,right=of coord,text width=29mm] (score) {Evaluate the observation-family posterior predictive};
\draw[arrPrimary] (post)--(cond);
\draw[arrPrimary] (cond)--(coord);
\draw[arrPrimary] (coord)--node[above,font=\scriptsize]{in support}(score);
\node[draw=Warning,fill=WarningPale,rounded corners,below=9mm of coord,text width=35mm,align=center] (err) {Outside support: reject unless an extrapolation model was specified before scoring};
\draw[arr,draw=Warning] (coord)--(err);
\node[neutralbox,below=9mm of score,text width=32mm] (match) {Boundary evaluation uses one-to-one matching; unmatched location error is NA};
\draw[arr] (score)--(match);
\end{tikzpicture}


==> shared/figures/tikz/workflows/scope_and_failure_map.tex <==
\begin{tikzpicture}[node distance=9mm and 12mm]
\node[primarybox,text width=32mm] (factor) {Contiguous partition with locally factorized segment contributions};
\node[primarybox,text width=32mm,right=of factor] (segment) {Finite segment marginal likelihood or stated numerical approximation};
\node[successbox,text width=32mm,right=of segment] (exact) {Exact partition recursion or conditional approximation bound};
\node[neutralbox,text width=34mm,below=14mm of factor] (nonlocal) {Nonlocal dependence among segments or unrestricted labels};
\node[neutralbox,text width=34mm,below=14mm of segment] (uncert) {Uncontrolled segment scores or observation-support mismatch};
\node[secondarybox,text width=34mm,below=14mm of exact] (outside) {Requires a different model, state space, or numerical analysis};
\draw[arrPrimary] (factor) -- (segment);
\draw[arrPrimary] (segment) -- (exact);
\draw[arr,dashed] (nonlocal) -- node[below,font=\scriptsize]{local factorization fails} (outside);
\draw[arr,dashed] (uncert) -- node[below,font=\scriptsize]{posterior interpretation not established} (outside);
\draw[arr,dashed] (factor) -- (nonlocal);
\draw[arr,dashed] (segment) -- (uncert);
\end{tikzpicture}


==> shared/figures/tikz/workflows/segment_to_partition.tex <==
\begin{tikzpicture}[node distance=8mm and 10mm]
\node[primarybox,text width=31mm] (data) {Ordered observations\\$u,y,d,a$};
\node[secondarybox,right=of data,text width=35mm] (segment) {Observation-model calculation\\$\log A^{(r)}_{ij}$};
\node[primarybox,above right=7mm and 13mm of segment,text width=32mm] (sum) {Sum-product recursion\\marginal likelihoods and posterior marginals};
\node[primarybox,below right=7mm and 13mm of segment,text width=32mm] (max) {Max-sum recursion\\joint MAP partition};
\node[successbox,right=13mm of sum,text width=31mm] (post) {$p(k\mid y)$, changepoint probabilities, Bayes curves};
\node[successbox,right=13mm of max,text width=31mm] (map) {Joint MAP changepoints and fitted segments};
\draw[arrPrimary] (data)--(segment);
\draw[arrPrimary] (segment)--(sum);
\draw[arrPrimary] (segment)--(max);
\draw[arrPrimary] (sum)--(post);
\draw[arrPrimary] (max)--(map);
\node[draw=Rule,dashed,rounded corners,fit=(sum)(max),inner sep=4mm,label=above:{\small dynamic programming over ordered partitions}] {};
\end{tikzpicture}


==> shared/figures/unified-system.tex <==
% Reusable TikZ diagram with no surrounding figure environment.
\newcommand{\CSUnifiedSystemDiagram}{%
\begin{tikzpicture}[
  node distance=7mm and 9mm,
  every node/.style={font=\rmfamily},
  source/.style={draw=Secondary,fill=SecondaryPale,rounded corners=2pt,
    minimum width=31mm,minimum height=11mm,align=center,line width=0.7pt},
  core/.style={draw=Primary,fill=PrimaryWash,rounded corners=2pt,
    minimum width=34mm,minimum height=13mm,align=center,line width=0.9pt},
  output/.style={draw=RuleDark,fill=white,rounded corners=2pt,
    minimum width=29mm,minimum height=10mm,align=center,line width=0.55pt},
  qa/.style={draw=Positive,fill=PositivePale,rounded corners=2pt,
    minimum width=41mm,minimum height=9mm,align=center,line width=0.7pt},
  flow/.style={-{Stealth[length=2.2mm]},draw=Ink,line width=0.75pt},
  feedback/.style={-{Stealth[length=2.2mm]},draw=Positive,dashed,line width=0.75pt},
]
  \node[source] (assets) {\textbf{Canonical research assets}\\[-1pt]
    \scriptsize metadata, figures, tables, code, references};
  \node[core,right=of assets] (system) {\textbf{Shared system layer}\\[-1pt]
    \scriptsize design tokens, notation, evidence labels};
  \node[output,right=13mm of system,yshift=12mm] (paper) {\textbf{Paper}\\[-1pt]
    \scriptsize dense, publication-facing};
  \node[output,right=13mm of system] (slides) {\textbf{Slides + notes}\\[-1pt]
    \scriptsize visual, claim-led};
  \node[output,right=13mm of system,yshift=-12mm] (book) {\textbf{Technical book}\\[-1pt]
    \scriptsize explanatory, pedagogical};
  \node[qa,below=13mm of system] (qa) {\textbf{Build and visual QA}\\[-1pt]
    \scriptsize compile, render, inspect, revise};

  \draw[flow] (assets) -- (system);
  \draw[flow] (system.east) -- ++(5mm,0) |- (paper.west);
  \draw[flow] (system.east) -- (slides.west);
  \draw[flow] (system.east) -- ++(5mm,0) |- (book.west);
  \draw[flow] (paper.south) -- ++(0,-4mm) -| (qa.east);
  \draw[flow] (slides.south) -- ++(0,-4mm) -| (qa.east);
  \draw[flow] (book.south) -- ++(0,-4mm) -| (qa.east);
  \draw[feedback] (qa.west) -| node[pos=0.25,left=1mm,font=\scriptsize\rmfamily,
    text=Positive]{revise once} (assets.south);
\end{tikzpicture}%
}


==> shared/saim/brand/colors.tex <==
% SAIM semantic color system - single source of truth.
% Load xcolor before inputting this file.

% Core brand colors derived from the supplied SAIM identity.
\definecolor{SAIMIndigo}{HTML}{32127A}
\definecolor{SAIMIndigoDark}{HTML}{1A0A40}
\definecolor{SAIMLavender}{HTML}{D6CFE4}
\definecolor{SAIMLavenderLight}{HTML}{F5F2FA}
\definecolor{SAIMInk}{HTML}{17131F}
\definecolor{SAIMDark}{HTML}{211934}
\definecolor{SAIMCoolGray}{HTML}{F4F2F8}
\definecolor{SAIMPanel}{HTML}{FAF9FC}
\definecolor{SAIMMuted}{HTML}{6F6879}
\definecolor{SAIMRule}{HTML}{D8D3E1}
\definecolor{SAIMRuleDark}{HTML}{978EA7}
\definecolor{SAIMBlue}{HTML}{2E5C8A}
\definecolor{SAIMBluePale}{HTML}{EAF2F8}
\definecolor{SAIMGreen}{HTML}{4A7A5C}
\definecolor{SAIMGreenPale}{HTML}{EAF3ED}
\definecolor{SAIMRed}{HTML}{A74455}
\definecolor{SAIMRedPale}{HTML}{F8EAEE}
\definecolor{SAIMAmber}{HTML}{9B6418}
\definecolor{SAIMAmberPale}{HTML}{FFF4DD}

% Semantic names shared by the paper, slides, lecture notes, book, and gallery.
% White remains the default page and component interior; lavender is reserved
% for selected emphasis, diagrams, and optional soft backgrounds.
\colorlet{Primary}{SAIMIndigo}
\colorlet{PrimaryDark}{SAIMIndigoDark}
\colorlet{PrimaryPale}{white}
\colorlet{PrimaryWash}{white}
\colorlet{Secondary}{SAIMBlue}
\colorlet{SecondaryPale}{SAIMBluePale}
\colorlet{Positive}{SAIMGreen}
\colorlet{PositivePale}{SAIMGreenPale}
\colorlet{Negative}{SAIMRed}
\colorlet{NegativePale}{SAIMRedPale}
\colorlet{Warning}{SAIMAmber}
\colorlet{WarningPale}{SAIMAmberPale}
\colorlet{Ink}{SAIMInk}
\colorlet{Muted}{SAIMMuted}
\colorlet{Rule}{SAIMRule}
\colorlet{RuleDark}{SAIMRuleDark}
\colorlet{CodeBackground}{SAIMCoolGray}
\colorlet{LightPanel}{SAIMPanel}

% Compatibility aliases retained from the supplied SAIM templates.
\colorlet{saimindigo}{Primary}
\colorlet{saimbg}{SAIMLavender}
\colorlet{saimfg}{Ink}
\colorlet{saimdark}{SAIMDark}
\colorlet{saimgray}{SAIMCoolGray}
\colorlet{saimblue}{Secondary}
\colorlet{saimgreen}{Positive}
\colorlet{saimlight}{SAIMLavenderLight}
\colorlet{lightblue}{SecondaryPale}
\colorlet{metablue}{Secondary}
\colorlet{metafg}{Ink}
\colorlet{metabg}{LightPanel}


==> shared/saim/brand/typography.tex <==
% SAIM Computer Modern Sans typography system - single source of truth.
% The system uses CMSS (regular), CMSSBX (bold), CMSSI (slanted), CMTT
% (monospaced), and the standard Computer Modern mathematics family. To
% prevent silent font drift, every target intentionally compiles with pdfLaTeX.
\RequirePackage{iftex}
\ifPDFTeX\else
  \PackageError{saim-typography}
    {The reference typography requires pdfLaTeX}
    {Select pdfLaTeX so the project uses the exact Computer Modern Sans and Computer Modern Math fonts.}
\fi

% Keep native OT1 Computer Modern encoding. pdfLaTeX
% embeds the Type 1 Computer Modern fonts supplied by the TeX distribution;
% no uploaded font files are required.
\RequirePackage[utf8]{inputenc}
\RequirePackage{fix-cm}
\RequirePackage[protrusion=true,expansion=true]{microtype}
\RequirePackage{setspace}

% CMSS is the dominant voice everywhere. Existing \rmfamily calls are mapped
% to CMSS as well, so paper, lecture notes, book, slides, captions, tables,
% diagrams, and running furniture remain typographically unified.
\renewcommand{\rmdefault}{cmss}
\renewcommand{\sfdefault}{cmss}
\renewcommand{\ttdefault}{cmtt}
\renewcommand{\familydefault}{\sfdefault}
\renewcommand{\itdefault}{sl}

% Semantic font roles.
\providecommand{\SAIMBodyFont}{\sffamily}
\providecommand{\SAIMHeadingFont}{\sffamily\bfseries}
\providecommand{\SAIMCoverTitleFont}{\sffamily\bfseries}
\providecommand{\SAIMCoverSubtitleFont}{\sffamily}
\providecommand{\SAIMNavigationFont}{\sffamily\bfseries}
\providecommand{\SAIMMetaFont}{\sffamily}
\providecommand{\SAIMCodeFont}{\ttfamily}

% Compatibility aliases used by the front-matter implementations.
\providecommand{\SAIMFrontFont}{\sffamily}
\providecommand{\SAIMFrontTitleFont}{\SAIMCoverTitleFont}
\providecommand{\SAIMFrontMetaFont}{\SAIMMetaFont}
\providecommand{\SAIMFrontRagged}{\raggedright\hyphenpenalty=10000\exhyphenpenalty=10000}


==> shared/saim/components/boxes.tex <==
% Shared tcolorbox vocabulary.
% Load tcolorbox with the `most` library before inputting this file.
\tcbset{
  saim/base/.style={
    enhanced,
    breakable,
    boxrule=0pt,
    arc=1.5pt,
    outer arc=1.5pt,
    left=8pt,
    right=8pt,
    top=7pt,
    bottom=7pt,
    before skip=8pt,
    after skip=8pt,
    fonttitle=\rmfamily\bfseries,
    coltitle=Ink,
    attach title to upper={\par\vspace{2pt}},
  },
  saim/primary/.style={
    saim/base,
    colback=PrimaryWash,
    borderline west={2.4pt}{0pt}{Primary},
    colframe=Primary,
  },
  saim/blue/.style={
    saim/base,
    colback=SecondaryPale,
    borderline west={2.4pt}{0pt}{Secondary},
    colframe=Secondary,
  },
  saim/green/.style={
    saim/base,
    colback=PositivePale,
    borderline west={2.4pt}{0pt}{Positive},
    colframe=Positive,
  },
  saim/amber/.style={
    saim/base,
    colback=WarningPale,
    borderline west={2.4pt}{0pt}{Warning},
    colframe=Warning,
  },
  saim/neutral/.style={
    saim/base,
    colback=LightPanel,
    borderline west={2.4pt}{0pt}{RuleDark},
    colframe=Rule,
  },
  saim/outline/.style={
    enhanced,
    breakable,
    colback=white,
    colframe=Rule,
    boxrule=0.55pt,
    arc=2pt,
    outer arc=2pt,
    left=8pt,
    right=8pt,
    top=7pt,
    bottom=7pt,
    before skip=8pt,
    after skip=8pt,
    fonttitle=\rmfamily\bfseries,
    coltitle=Ink,
  },
}


==> shared/saim/components/evidence.tex <==
% Compact evidence-status labels usable in paper, slides, and book.
% Requires xcolor; no other package dependency.
\newcommand{\SAIMEvidenceTag}[3]{%
  \begingroup
  \setlength{\fboxsep}{2.6pt}%
  \setlength{\fboxrule}{0.45pt}%
  \raisebox{0.2ex}{\fcolorbox{#1}{#2}{%
    \textcolor{#1}{\sffamily\bfseries\fontsize{7}{8}\selectfont\strut\MakeUppercase{#3}}}}%
  \endgroup}
\newcommand{\MeasuredTag}{\SAIMEvidenceTag{Positive}{PositivePale}{Measured}}
\newcommand{\ReproducedTag}{\SAIMEvidenceTag{Secondary}{SecondaryPale}{Reproduced}}
\newcommand{\SyntheticTag}{\SAIMEvidenceTag{Warning}{WarningPale}{Synthetic}}
\newcommand{\PlannedTag}{\SAIMEvidenceTag{RuleDark}{LightPanel}{Planned}}
\newcommand{\IllustrativeTag}{\SAIMEvidenceTag{PrimaryDark}{PrimaryWash}{Illustrative}}
\newcommand{\ExternalTag}{\SAIMEvidenceTag{Secondary}{SecondaryPale}{External}}


==> shared/saim/components/frontmatter.tex <==
% Shared front-page typography roles.
% Computer Modern Sans is used for titles, metadata, navigation, and prose,
% matching the attached reference deck. Computer Modern Typewriter remains
% reserved for code and technical literals.
\providecommand{\SAIMFrontFont}{\sffamily}
\providecommand{\SAIMFrontTitleFont}{\SAIMCoverTitleFont}
\providecommand{\SAIMFrontMetaFont}{\SAIMMetaFont}
\providecommand{\SAIMFrontRagged}{\raggedright\hyphenpenalty=10000\exhyphenpenalty=10000}


==> shared/saim/components/listings.tex <==
% Shared code-listing styles. Load listings before inputting this file.
\lstdefinestyle{python}{
  language=Python,
  basicstyle=\ttfamily\small\color{Ink},
  keywordstyle=\color{PrimaryDark}\bfseries,
  stringstyle=\color{Positive},
  commentstyle=\color{Muted}\itshape,
  numberstyle=\scriptsize\color{RuleDark},
  numbers=left,
  numbersep=9pt,
  backgroundcolor=\color{CodeBackground},
  frame=leftline,
  rulecolor=\color{Primary},
  framerule=1.4pt,
  breaklines=true,
  showstringspaces=false,
  keepspaces=true,
  columns=fullflexible,
  xleftmargin=12pt,
  framexleftmargin=4pt,
  aboveskip=9pt,
  belowskip=9pt,
  captionpos=t,
}
\lstdefinestyle{console}{
  basicstyle=\ttfamily\small\color{Ink},
  backgroundcolor=\color{LightPanel},
  frame=leftline,
  rulecolor=\color{Secondary},
  framerule=1.4pt,
  breaklines=true,
  columns=fullflexible,
  xleftmargin=12pt,
  framexleftmargin=4pt,
  aboveskip=9pt,
  belowskip=9pt,
  captionpos=t,
}


==> shared/saim/components/math.tex <==
% =============================================================================
% math.tex - shared project notation
% =============================================================================
% Do not load packages here. The document entrypoints load amsmath, amssymb,
% amsfonts, amsthm, mathtools, and any project-specific dependencies.

% Number sets and expectations
\providecommand{\R}{\mathbb{R}}
\providecommand{\E}{\mathbb{E}}

% Common operators
\providecommand{\KL}{\operatorname{KL}}
\providecommand{\DKL}{D_{\mathrm{KL}}}
\providecommand{\Var}{\operatorname{Var}}
\providecommand{\Cov}{\operatorname{Cov}}
\providecommand{\argmax}{\operatorname*{arg\,max}}
\providecommand{\argmin}{\operatorname*{arg\,min}}

% Delimiters
\providecommand{\norm}[1]{\left\lVert #1 \right\rVert}
\providecommand{\abs}[1]{\left\lvert #1 \right\rvert}
\providecommand{\set}[1]{\left\{ #1 \right\}}
\providecommand{\paren}[1]{\left( #1 \right)}
\providecommand{\bracket}[1]{\left[ #1 \right]}
\providecommand{\ip}[2]{\left\langle #1, #2 \right\rangle}

% Example policy notation. Delete or extend for a different project.
\providecommand{\pitheta}{\pi_{\theta}}
\providecommand{\piref}{\pi_{\mathrm{ref}}}
\providecommand{\pistar}{\pi^{*}}


==> shared/saim/components/tikz.tex <==
% Shared TikZ vocabulary for paper, slides, and book.
% Load tikz and the required libraries before inputting this file.
\tikzset{
  arrow/.style={-{Stealth[length=2.5mm]}, thick, saimdark},
  darrow/.style={-{Stealth[length=2.5mm]}, thick, dashed, saimdark},
  csblock/.style={rectangle, rounded corners=2pt, thick, fill=saimbg, text=saimdark,
                  minimum height=1.0cm, minimum width=3.6cm, align=center,
                  font=\small\rmfamily},
  csfinal/.style={rectangle, rounded corners=2pt, thick, fill=saimindigo, text=white,
                  minimum height=1.0cm, minimum width=3.6cm, align=center,
                  font=\small\rmfamily},
  cslevel1/.style={rectangle, rounded corners=2pt, fill=saimindigo, text=white,
                   text width=9em, text centered, minimum height=2.2em,
                   font=\small\rmfamily\bfseries},
  cslevel2/.style={rectangle, rounded corners=2pt, fill=saimbg, text=saimdark,
                   text width=7.5em, text centered, minimum height=1.8em,
                   font=\scriptsize\rmfamily},
  cscrosscut/.style={rectangle, rounded corners=2pt, fill=saimgray, text=saimdark,
                     draw=saimblue, dashed, text width=8em, text centered,
                     minimum height=1.8em, font=\scriptsize\rmfamily},
  csmethodbox/.style={rectangle, fill=saimindigo, text=white, minimum width=2.6cm,
                      minimum height=0.8cm, font=\small\rmfamily\bfseries,
                      text centered},
  cspropbox/.style={rectangle, fill=saimbg, text=saimdark, minimum width=2.6cm,
                    minimum height=0.6cm, font=\scriptsize\rmfamily,
                    text centered, text width=2.6cm},
  csstagelbl/.style={font=\rmfamily\bfseries\small, text=saimindigo},
  boxbase/.style={draw,rounded corners=2pt,minimum height=9mm,align=center,
                  line width=0.6pt,font=\small\rmfamily,inner sep=5pt},
  primarybox/.style={boxbase,fill=PrimaryPale,draw=Primary},
  secondarybox/.style={boxbase,fill=SecondaryPale,draw=Secondary},
  neutralbox/.style={boxbase,fill=black!3,draw=Rule},
  successbox/.style={boxbase,fill=Positive!10,draw=Positive},
  arr/.style={-{Stealth[length=2.2mm]},line width=0.7pt,draw=Ink},
  arrPrimary/.style={-{Stealth[length=2.2mm]},line width=0.9pt,draw=Primary},
  arrSecondary/.style={-{Stealth[length=2.2mm]},line width=0.9pt,draw=Secondary},
  tier/.style={draw=Rule,rounded corners=4pt,dashed,line width=0.5pt,inner sep=3mm}
}


==> shared/tables/defs/tab_nonconj_tradeoff.tex <==
\begin{table}[!htbp]
\centering
\scriptsize
\resizebox{0.97\textwidth}{!}{\input{shared/tables/results/table4_nonconj_tradeoff.tex}}
\caption{Local approximation comparison. The observed maximum errors are too large to treat this example as verification of a small uniform segmentwise error bound.}
\label{tab:nonconjugate-result-paper}
\end{table}


==> shared/tables/defs/tab_runtime_result.tex <==
\begin{table}[!htbp]
\centering
\small
\input{shared/tables/results/table1_runtime_scaling.tex}
\caption{Runtime measurements for $k_{\max}=20$ in the length sweep.}
\label{tab:runtime-result-paper}
\end{table}


==> shared/tables/evaluation-plan.tex <==
\begin{table}[htbp]
\centering
\caption{Evaluation matrix. All example outcomes are \textbf{(PLANNED)} and
must be replaced by measured values before publication.}
\label{tab:evaluation-plan}
\small
\renewcommand{\arraystretch}{1.25}
\begin{tabularx}{\textwidth}{@{}L{0.17\textwidth}L{0.21\textwidth}L{0.21\textwidth}Y@{}}
\toprule
Claim & Metric & Baseline & Decision rule \\
\midrule
Higher task quality & Primary task score & Strongest matched system &
Improvement exceeds the predeclared uncertainty margin \\
Lower resource cost & Peak memory, latency, energy & Same quality operating point &
Cost reduction persists under realistic load \\
Mechanism is necessary & Ablation delta & Full proposed system &
Removing the component degrades the predicted quantity \\
Robust under shift & Worst-group or stress score & In-distribution result &
Degradation remains within the deployment tolerance \\
\bottomrule
\end{tabularx}
\end{table}


==> shared/tables/results/tab_E06_approx.tex <==
\begin{table}[ht]
\centering
\caption{Nonconjugate block-evidence approximations. Block sizes $B\in\{4,8,16,32,64,128\}$,
$p\in\{0.05,0.5,0.95\}$, 100 independent replicates per cell (1800 blocks total).
Prior $\theta\sim\mathcal{N}(0,4)$. Reference: Gauss--Hermite quadrature with $Q=200$ nodes.
\texttt{pg\_vb} is an alias of JJ and is not listed separately.
JJ LB rate: fraction of blocks where JJ $\le$ reference $+$ \num{1e-8}.
EP is \emph{not} a guaranteed lower bound.}
\label{tab:planned-nonconjugate-paper}
\begin{tabular}{lrrrrr}
\toprule
Method & Median $|\Delta\log Z|$ & Max $|\Delta\log Z|$ & JJ LB violations & EP failures & Median runtime \\
\midrule
  Laplace & 0.0208 & 0.0377 & N/A & --- & 0.050ms \\
  JJ (= pg\_vb alias) & 0.2225 & 0.9769 & 0/1800 & --- & 0.235ms \\
  EP & 3.7788 & 30.0009 & N/A & 0/1800 & 2.093ms \\
\bottomrule
\end{tabular}
\end{table}


==> shared/tables/results/table1_runtime_scaling.tex <==
\begin{tabular}{rrrr}\toprule
n & $k_{\max}$ & mean (s) & std (s)\\\midrule
50 & 20 & 0.0750 & 0.0026\\
100 & 20 & 0.1631 & 0.0019\\
200 & 20 & 0.3725 & 0.0172\\
400 & 20 & 0.7721 & 0.0047\\
\bottomrule\end{tabular}


==> shared/tables/results/table4_nonconj_tradeoff.tex <==
\begin{tabular}{lrrrrrr}\toprule
Method & $\max|\Delta \log A^0|$ & $q_{95}|\Delta \log A^0|$ & median $|\Delta \log A^0|$ & time (s) & F1@$\tau$ & $\hat{k}$\\\midrule
quadrature & 0.000 & 0.000 & 0.000 & 0.146 & 0.500 & 3\\
laplace & 1.235 & 1.188 & 0.980 & 0.079 & 0.500 & 3\\
jj & 1.265 & 1.216 & 1.002 & 0.169 & 0.500 & 3\\
ep & 1.631 & 1.407 & 0.939 & 4.379 & 0.364 & 10\\
pg-vb & 1.265 & 1.216 & 1.002 & 0.160 & 0.500 & 3\\
\bottomrule\end{tabular}

